A Stable Measure of Similarity for Time Series using Persistent Homology

Persistent homology, the study of holes that appear in data as one thickens balls centered around its points over time, has theoretically guaranteed stability. That is, small data perturbations guarantee small changes in the lifetimes of these holes. This stability has been used to construct a measure of periodicity for a single univariate time series, denoted score(f1). One popular measure of similarity between two time series is percent determinism (%DET), which measures the correlation between two time-series embeddings. We introduce a novel persistent-homology based measure of time-series similarity which we denote the bi-conditional periodicity score, score(f1,f2). We prove the stability of our measure under small time series and frequency perturbations, as well as the existence of a minimum embedding dimension for the convergence of our score. Our latter result implies that larger embedding dimensions may be necessary to reach desired levels of convergence. Since pairwise distances between points in these larger dimensions may start to concentrate, we also prove the stability of our measure under dimension reduction which guarantees that as long as the first K principal components capture a majority of the variance under orthogonal projection, the score will undergo small changes. We next introduce an algorithm for computing the bi-conditional periodicity score and deduce its computational complexity as O(N log N + PK^2 + P^6) for N the number of time series points, P the number of embedding points, and K the number of principal components. We experimentally verify the greater stability of our measure in comparison with %DET on both synthetic time series as well as real climate data. As well, score(f1,f2) requires only one parameter for its computation while %DET requires four.

==> def.tex <==
\section{Definitions}\label{sec:def}

\subsection{Persistent Homology}

Here we introduce standard definitions of topological features used in this paper. 
More information can be found in \cite{Munkres1984,OtPoTiGrHa2017}.

\begin{definition}
    [Vietoris-Rips Complex]\label{def:VR_cmplx}
    Given a point cloud $X = \{x_1,x_2,\dots,x_n\} \in \vR^d$ and a filtration radius $\epsilon > 0$, the Vietoris-Rips complex of $X$ at $\epsilon$ is given by the collection of simplices below

    \[ \mathcal{R}_\epsilon(X) = \{ \sigma = [x_i \dots x_j] : i,j \in 1 \dots n; ||x_s - x_k|| \leq 2 \epsilon, s,k \in 1 \dots n \}. \]
\end{definition}

\begin{definition}
    [Vietoris-Rips Filtration]\label{def:VR_filtrn}
    Given a collection of increasing filtration radii $0 = \epsilon_1 < \epsilon_2 < \dots < \epsilon_r < \dots$ applied to a point cloud $X$, the collection of nested subcomplexes 

    \[ X \subset \mathcal{R}_{\epsilon_2}(X) \subset \dots \subset \mathcal{R}_{\epsilon_r}(X) \subset \dots \]

    \noindent denotes the Vietoris-Rips filtration of $X$, given by $\mathcal{R}(X)$.
\end{definition}

%\begin{definition}
 %   [Sublevel-set of a Function]\label{def:sublevel_set}
 %   Let $f : \vR \rightarrow \vR$ be a continuous tame function. 
 %   Then the sublevel-set of $f$ at level $\lambda$ is given by 

 %   \[ \mathcal{S}_\lambda(f) = \{ f(x) : f(x) \leq \lambda \}. \]
%\end{definition}

%\begin{definition}
%    [Sublevel-set Filtration]\label{def:sublevel_set_filtrn}
%    Given a collection of increasing sublevel-set values $\lambda_1 < \lambda_2 < \dots < \lambda_v < \dots$ applied to a continuous tame function $f: \vR \rightarrow \vR$, the collection of nested sublevel-sets 
%
%    \[ \mathcal{S}_{\lambda_1}(f) \subseteq \mathcal{S}_{\lambda_2}(f) \subseteq \dots \subseteq \mathcal{S}_{\lambda_v}(f) \subseteq \dots \]

%    \noindent denotes the sublevel-set filtrtaion of $f$, given by $\mathcal{S}(f)$.
%\end{definition}

\begin{definition}
    [Persistence Diagram]\label{def:dgm}
    Given Vietoris-Rips filtration on a point cloud $X$, the collection of birth and death radii for each $p$-dimensional hole that appears can be summarized as ordered pairs in a persistence diagram given below by 

    \[ \dgm(\mathcal{R}(X)) = \{ (b_i,d_i):i=1,\dots,m_p,p=0,1,2,\dots\}. \]

    %\noindent Similarly, given sublevel-set filtration of a continuous function $f: \vR \rightarrow \vR$, the persistence diagram can be denoted by 

    %\[ \dgm(\mathcal{S}(f)) = \{ (b_i,d_i):i=1,\dots,m_0 \}.\]
    
    \noindent Unless otherwise stated, we simplify this notation to $\dgm(X)$, denoting $\dgm_p(X)$ as the collection of all ordered pairs for one dimension $p$ from $\dgm(X)$.
\end{definition}

\begin{definition}
    [Persistence Barcode]\label{def:bcd}
    Given Vietoris-Rips filtration on a point cloud $X$, the collection of birth and death radii for each $p$-dimensional hole that appears can be summarized as intervals in a persistence barcode given  below by

    \[ \bcd(\mathcal{R}(X)) = \{ [b_i,d_i):i=1,\dots,m_p,p=0,1,2,\dots\}. \]

    %\noindent Similarly, given sublevel-set filtraiton of a continuous function $f: \vR \rightarrow \vR$, the persistence barcode can be denoted by 

    %\[ \bcd(\mathcal{S}(f)) = \{ [b_i,d_i) : i = 1, \dots, m_0 \}. \]

    \noindent Unless otherwise stated, we simplify this notation to $\bcd(X)$, denoting $\bcd_p(X)$ as the collection of all intervals for one dimension $p$ from $\bcd(X)$.
\end{definition}

\subsection{Distance Metrics}

Here we introduce standard definitions of distances used in this paper.
See, for instance, the book by Burago, Bugaro, and Ivanov~\cite{BuBuIv2001} for details. 

%\begin{definition}
 %   [Infinity Norm]\label{def:infty_norm}
 %   Define two continuous real-valued functions $f$ and $g$. 
 %   The infinity norm of their difference is denoted 

 %   \[ ||f-g||_\infty = \max_x \{ | f(x) - g(x) | \}. \]
%\end{definition}

\begin{definition}[Hausdorff Distance]\label{def:Hausdorf_dist}
  Given two sets of points $X$ and $Y$ in a common metric space, the Hausdorff distance between them is given by 
  \[\dH(X,Y) = \inf{\{\epsilon>0:X \subseteq Y^{\epsilon}, Y \subseteq X^{\epsilon}\}}, ~\text{ where }
  X^{\epsilon} = \underset{x \in X}{\bigcup} B_{\epsilon}(x) \text{ and } Y^{\epsilon}= \underset{y \in Y}{\bigcup} B_{\epsilon}(y)\]
  denote the union of all $\epsilon$-balls centered at each point in either set. 
\end{definition}

\begin{definition}[Hausdorff Definition of Gromov-Hausdorff Distance]\label{def:Gromov_Hausdorf_dist_Hausdorf}
  Given two sets of points $X$ and $Y$, the Gromov-Hausdorff distance between them is given by 
  \[ \dGH(X,Y) = \inf{\{\dH(f(X),g(Y)) : f:X\rightarrow S, g:Y\rightarrow S \}}, \]
  where $f$ and $g$ are isometric embeddings of $X$ and $Y$ into a common metric space $S$.
  If $X$ and $Y$ lay in a shared metric space $S$,  then $\dGH(X,Y) \leq \dH(X,Y)$ \cite{adams2024}.
\end{definition}

\begin{definition}[Distortion Definition of Gromov-Hausdorff Distance]\label{def:Gromov_Hausdorf_dist_distortion}
  An alternative definition of the Gromov-Hausdorff distance between two sets of points $X$ and $Y$ is given by 
  \[ \dGH(X,Y) = \frac{1}{2} \inf{\{\dis(R):R:X\rightarrow Y} \in \mathcal{R}(X,Y)\}, \]
  where $R$ is a relation between $X$ and $Y$ whose distortion is defined by 
  \[ \dis(R) = \sup \{|d_X(x,x') - d_Y(y,y')| \,:\, (x,y), (x',y') \in R\},\]
  where $d_{X}$ and $d_{Y}$ are the corresponding metrics for $X$ and $Y$, respectively. 
\end{definition}

\begin{definition}[Bottleneck Distance]\label{def:Bottleneck_dist}
  Given two finite sets of points $X$ and $Y$, let $\dgm(X)$ and $\dgm(Y)$ denote the persistence diagrams of a chosen dimension obtained from the Vietoris-Rips (VR) filtration on $X$ and $Y$, respectively.
  Then the Bottleneck distance between $\dgm(X)$ and $\dgm(Y)$ is given by 
  
  \[ \dB(\dgm(X),\dgm(Y)) = \underset{\phi}{\inf}\,\underset{x}{\sup} \norm{x - \phi(x)}_{\infty}, \]
  
  \noindent where $\phi:\dgm(X) \rightarrow \dgm(Y)$ denotes a bijection between $\dgm(X)$ and $\dgm(Y)$, including points along the diagonal in either diagram when they both do not share the same cardinality.
  %Similarly, the Bottleneck distance between the persistence diagrams obtained from sublevel-set filtration on the continuous tame functions $f, g : \vR \rightarrow \vR$ is defined equivalently, which we denote 
  
  %\[ \dB(\dgm(f),\dgm(g)) = \underset{\phi}{\inf}\,\underset{x}{\sup} \norm{x - \phi(x)}_{\infty}. \]
\end{definition}

\subsection{The Conditional Periodicity Scoring Function}

Here we denote the definitions for our new scoring function.

\begin{definition}
    [Conditional Sliding Windows Embedding]\label{def:conditional_SWE}
    Given a continuous univariate time series $f_1:T \subseteq \vR \rightarrow \vR$ and a reference series $f_2$ with a frequency of $w_2 = \arg\max_w \left\vert \int_T f_2(t) e^{i 2 \pi w t}dt \right\vert$ Hertz (Hz) (i.e. cycles per second), define the time lag $\tau_{w_2} = \frac{1}{w_2(M+1)}$ for embedding dimension $M \in \vN$. 
    Then the conditional sliding windows embedding of $f_1$ given $f_2$ is given by 

    \[ \SW_{M,\tau_{w_2}} f_{1|2}(t) = (f_1(t),f_1(t+\tau_{w_2}), \dots, f_1(t+M\tau_{w_2})). \]
\end{definition}

\begin{definition}
    [Conditional Periodicity Score]\label{def:conditional_score}
    Denote the lifetime of the longest-surviving 1-dimensional hole from Vietoris-Rips filtration on the conditional sliding windows embedding of a continuous time series $f_1$ given a reference series $f_2$ with frequency $w_2 = \arg\max_w \left\vert \int_T f_2(t) e^{i 2\pi w t}dt \right\vert$ Hz by $\mp(\dgm_1(\SW_{M,\tau_{w_2}}f_{1|2}(T)))$.
    Then the conditional periodicity score of $f_1$ given $f_2$ is given by the normalization of this lifetime below:

    \[ \score(f_1|f_2) = \frac{\mp(\dgm_1(\SW_{M,\tau_{w_2}}f_{1|2}(T)))}{\sqrt{3}}. \]
\end{definition}

\begin{definition}
    [Bi-Conditional Periodicity Score]\label{def:bi_conditional_score}
    Given a continuous univariate time series $f_1 : T_1 \subseteq \vR \rightarrow \vR$ and a reference series $f_{2} : T_2 \subseteq \vR \rightarrow \vR$, denote the frequency of each signal as $w_1 = \arg\max_w \left\vert \int_{T_1}f_1(t) e^{i 2 \pi  w t} dt \right\vert$ and $w_2 = \arg\max_w \left\vert \int_{T_2}f_2(t) e^{i 2 \pi  w t} dt \right\vert$.
    Given time lags $\tau_{w_1} = \frac{1}{w_1(M+1)}$ and $\tau_{w_2} = \frac{1}{w_2(M+1)}$, the bi-conditional periodicity score of $f_1$ and $f_2$ is given by 

    \[ \score(f_1,f_2) = \frac{\score(f_1|f_2) + \score(f_2|f_1)}{2}. \]
\end{definition}
